Towards Automatic Threat Detection: A Survey of Advances of Deep Learning within X-ray Security Imaging

X-ray security screening is widely used to maintain aviation/transport security, and its significance poses a particular interest in automated screening systems. This paper aims to review computerised X-ray security imaging algorithms by taxonomising the field into conventional machine learning and contemporary deep learning applications. The first part briefly discusses the classical machine learning approaches utilised within X-ray security imaging, while the latter part thoroughly investigates the use of modern deep learning algorithms. The proposed taxonomy sub-categorises the use of deep learning approaches into supervised, semi-supervised and unsupervised learning, with a particular focus on object classification, detection, segmentation and anomaly detection tasks. The paper further explores well-established X-ray datasets and provides a performance benchmark. Based on the current and future trends in deep learning, the paper finally presents a discussion and future directions for X-ray security imagery.

==> lib/packages.tex <==
\usepackage{times}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{subfig}
% \usepackage{authblk}
\usepackage{csquotes}
\usepackage{graphics,graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{lipsum}
\usepackage{booktabs, multirow}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
% \usepackage{landscape}
% CAPTION & REF
\usepackage[pagebackref, colorlinks]{hyperref}
\usepackage{cite}

\usepackage{todonotes}
\setlength{\marginparwidth}{1.2cm}  % FTODO fit

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\usepackage{url}
\def\UrlBreaks{\do\/\do-} % Break long URLs in ref.

% Self-defined functions.
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\etal}{\emph{et al. }}
\newcommand{\sota}{state-of-the-art }
\newcommand{\ssection}[1]{\noindent{\textbf{#1.}}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

\usepackage{filecontents}
\usepackage{tikz}
\usepackage{tikz-qtree}
\usetikzlibrary{trees} 
\usepackage{pdflscape}
\usepackage{rotating}

% \pgfplotsset[compat=1.15]

% Resolve Unicode erros.
\usepackage{newunicodechar}
\newunicodechar{ﬁ}{fi}
\newunicodechar{ﬀ}{ff}

% TIKZ
\usetikzlibrary{arrows.meta,angles,quotes}
\colorlet{linecol}{black!75}
\usepackage{forest}
\tikzset{
  my rounded corners/.append style={rounded corners=2pt},
}

% COLOR
\usepackage{xcolor}

==> tex/0.front-matter.tex <==
\title{
    Towards Automatic Threat Detection: A Survey of Advances of Deep Learning within X-ray Security Imaging
}

\author{
	Samet~Akcay\textsuperscript{*},
	and~Toby~P.~Breckon \vspace{-0.5cm}
	\thanks{
		S. Akcay\textsuperscript{*}, TP. Breckon are with Department of Computer Science, Durham University, Durham, UK (e-mail: \{
			\href {mailto:samet.akcay@durham.ac.uk}{samet.akcay}, 
			\href {mailto:toby.breckon@durham.ac.uk}{toby.breckon}
		\}@durham.ac.uk).
	}
	\thanks{\textit{Asterisk indicates corresponding author}.}	
}

\maketitle
\begin{abstract}
    Having shown promising performance on challenging domains in computer vision, deep learning has also become a common trend in the X-ray security domain. This paper aims to review the current X-ray security literature by taxonimizing the traditional machine learning and contemporary deep learning approaches applied in the field.  The review presented here analyzes more than [NUMBER] of papers from various tasks such as classification, detection, and segmentation. The analysis provides substantial evidence that the applicability of deep learning algorithms in this domain is rather promising. Based on the current and future trends in deep learning, the paper finally presents a discussion and future directions for X-ray security imagery. 
\end{abstract}





==> tex/7.references.tex <==
% - - - - - - - - - - - - - - - - - - - - %
% References                              %
% - - - - - - - - - - - - - - - - - - - - %

{    
    \bibliographystyle{IEEEtran}
    \small
    \bibliography{ref/library.bib}
}

==> tex/A.dl-theory.tex <==
% - - - - - - - - - - - - - - - - - - - - %
% Deep Learning in X-ray Security Imaging %
% - - - - - - - - - - - - - - - - - - - - % 
\section{Deep Learning Approaches within X-ray Security Imaging}
\label{sec:dl.approaches}
This section briefly introduces the recent deep learning approaches employed within X-ray security domain. It is important to note that the scope of the deep learning approaches discussed here is limited to those only used in X-ray security imaging. 

\subsection{A Background on Neural Networks}
\label{subsec:dl.background}
 A multi-layer perceptron $f$, one of the fundamental neural network approaches, consists of a single layer $h$ or stack of $n$ multiple layers $\mathbf{h}=\{h_0, h_1, \ldots h_n\}$, each of which comprises of set of neurons, activations ($a$) and non-linear transformation ($\sigma$). An activation of a layer $i$, denoted as $a^{(i)}$ is the linear combination of the input $\mathbf{x}^{(i-1)}$ and parameters $\theta^{(i)}=\{\mathbf{W}^{(i)}, b^{(i)}\}$, where $\mathbf{W}^{(i)}$ and $b^{(i)}$ are the weights and the biases such that $a^{(i)} = \mathbf{w_i^Tx^{(i-1)}} + b^{(i)}$. The $i^{th}$ layer $h^{(i)}$ is a function, where a non-liner transformation $\sigma^{(i)}$ is applied to the activation $a^{(i)}$ such that $h^{(i)} = \sigma^{(i)}(a^{(i)})$. Hence, the output of the $i^{th}$ layer is $h^{(i)}=\sigma^{(i)}(\mathbf{w_{i}^Tx} + b)$. 
 
 Overall, an $n$ layer network, comprises of $n$ hidden layers, where $\mathbf{h}=\{h_0, h_1, \ldots h_n\}$, and parameters $\Theta = \{ \mathcal{W}, \mathcal{B} \} $, where $\mathcal{W} = \{ \mathbf{w_1}, \mathbf{w_2}, \ldots, \mathbf{w_n} \}$ and $\mathcal{B} = \{b_1, b_2, \ldots, b_n\}$. The overall network $f$ is the composition of the hidden layers such that
 
 \begin{equation}
     f(\mathbf{x}; \Theta) = f(h_n \circ \ldots \circ h1\circ h_0)
 \end{equation}


% SOFTMAX
The final layer $h^{(n)}$ of the model $f$ outputs $C$ vectors, where $C$ is the number of the classes within the dataset $\mathcal{D}$. 

For an $n$ layer network $f$, the output activation is $a^{(n)} = \mathbf{w}_n^T \mathbf{x}^{(n-1)} + b^{(n)}$. For a simpler notation let $z = a^{(n)}$. The network outputs $C$ vectors $\mathbf{z} = \{z_1, z_2, \ldots, z_C\}$, where $C$ is the number of classes, and each $z$ is the feature encoding for class $j$. The next step is to classify the input $x$, based on its feature encoding $\mathbf{z}$. Softmax is the most common function used to classify the feature encoding in neural networks. A Softmax function takes an input feature encoding $\mathbf{z}$, and returns a probabilistic output, representing the likelihood of the input belonging to class $j$. Hence, the softmax output of $z$ for class $j$ is

\begin{equation}
    P(y_j | \mathbf{x}; \Theta) = \sigma(z)_j = \dfrac{e^{z_j}}{\sum_{c=1}^{C} e^{z_c}}, \quad j = 1, \ldots, C.
\end{equation}

Recall from Section \ref{sec: introduction} that the performance of a task is optimized via a loss function. In a classification task, for instance, cross entropy is used to measure the performance of the probabilistic output of the softmax function. Cross-entropy, also known as log-loss, penalizes the model as the predicted probability deviates from the ground-truth. The mathematical definition of this loss function is as follows:

\begin{equation}
   \mathcal{L} = \argmin_{\Theta} \Big( -\sum_{c=1}^{C} y_{c} log(p_{c})\Big),
\end{equation}
where $y_c$ is a binary label indicating whether the label c is correct for the sample, and $p_c$ is the probability predicted for the class $c$ by softmax.


\subsection{Convolutional Neural Networks -- CNN}
\label{subsubsec:dl.approaches.cnn}
Convolutional neural networks (CNN) are considered to be modern neural networks with key distinctions. Unlike MLPs that connect all neurons to other neurons, which is impractical, CNN uses local receptive fields, also known as filter or kernels, that spatially connect neurons to their local region. The use of local receptive fields makes CNN equivariant to image translations. Each layer $h$ consists of $K$ kernels with weights $\mathbf{\mathcal{W}} = \{\mathbf{w_1}, \mathbf{w_2}, \ldots, \mathbf{w_K}\}$ and biases $\mathcal{B} = \{b_1, b_2, \ldots, b_K\}$.  The second major difference is weight sharing that shares weights of the filters $\mathcal{W}$ across individual feature map of each layer $h$. Weight sharing radically decreases the number of parameters needed to train a deep neural network. 

\begin{figure}[ht]
    \centering
    \includegraphics{img/cnn_basic.pdf}
    \caption{Caption}
    \label{fig:basic-cnn}
\end{figure}

Another difference is that, within the network, convolutional layers are usually followed by pooling layers which down-samples the current representation (image) and hence reduces the number of parameters carried forward in-addition to improving overall computational efficiency.  

\begin{figure}[ht]
    \centering
    \includegraphics{img/dropout.pdf}
    \caption{Application of dropout, whereby the neurons are randomly removed from the network to avoid over-fitting.}
    \label{fig:dropout}
\end{figure}

The high-level of parametrization, and hence representational capacity, make CNN susceptible to over-fitting in the traditional sense. The use of dropout, whereby hidden neurons are randomly removed during the training process, is used to avoid over-fitting such that performance dependence on individual network elements is reduced in favor of cumulative error reduction and representational responsibility for the problem space. 

% \todo[inline]{ReLu here.}

The design of deep CNN poses instability issues during training. The use of BatchNorm \cite{Ioffe2015}, whereby its non-linearity normalizes the input for each hidden layer resolves the stability issues. For the $i^{th}$ hidden layer $h^{(i)}$, the output of the layer would typically be

\begin{align}
    x^{(i)} &= \sigma_i(\mathbf{w_i^T}x^{(i-1)}) \\ \notag
            &= \sigma_i(a^{(i)})
\end{align}
where $\sigma$ is the non-linearity function, and $\mathbf{w_i^T}x^{(i-1)}$ is activation $a^{(i)}$. BatchNorm normalizes the activation $a^{(i)}$ such that

\begin{equation}
    \tilde{a}^{(i)} = \dfrac{a^{(i)} \mathbb{E}[a^{(i)}]}{\sqrt{\mathbb{V}[a^{(i)}]}},
\end{equation}

where $\mathbb{E}[a^{(i)}]$ and  $\mathbb{V}[a^{(i)}]$ are the mean and the variance of the activation $a^{(i)}$, respectively. Normalizing the layers outputs based on the above equations minimizes the massive gradients during the optimization, and hence leads to faster convergence. 
All of the unique differences of CNN listed above make them much more efficient and reliable compared to traditional MLP. The following subsections introduce renown CNN strategies proposed for classification, detection, segmentation, and also applied within X-ray security imaging.


\subsection{Supervised CNN Architectures}
\label{sec:dl.approaches.cnn.architectures}


\subsubsection{Classification Architectures}
\label{sec:dl.approaches.cnn.classification}
This section explores the contemporary classification strategies proposed during the deep learning erea, and applied wihtin X-ray security imaging.



\paragraph{AlexNet}
\label{model.alexnet}
Similar to \cite{Lecun1998} but deeper and wider, this network is of 5 $ conv $ layers with  $ 11 \times 11 $  receptive filters and 3 $ fc $ layers, and 60 million parameters in total. To eliminate the network's susceptibility to over-fitting, caused by the high number of parametrization, the network employs the use of dropout, by randomly removing neurons during the training. Besides, the network utilizes ReLUs for non-linearity to accelerate the training process. figure \ref{fig:cnn.pipeline} demonstrates the overall pipeline of the architecture. 

\paragraph{VGG}
\label{model.vgg}
Following the AlexNet's breakthrough within the field, Simonyan and Zisserman (VGG) \cite{Simonyan2014} investigate the depth on classification performance by designing CNN via stacking convolutional layers with small $3 \times 3$ receptive fields with a stride of $1$. Small receptive fields increase non-linearity of the network but decrease the total number of the parameters of the network. This design choice is shown to improve state-of-the-art significantly. figure \ref{fig:cnn.pipeline} depicts the overall pipeline of the architecture, similar to \hyperref[model.alexnet]{AlexNet}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{img/vgg16.pdf}
    \caption{Caption}
    \label{fig:cnn.pipeline}
\end{figure}


\paragraph{ResNet}
\label{model.resnet}
Proposed by He \etal \cite{He2015}, this architecture is also designed to train deeper networks via its residual connections. The difficulty of training deep networks is that the training becomes unstable as the network goes deeper, which is due to losing the gradients of the input. He \etal propose a residual connection approach that forward-passes input to a stack of two convolutional layers (residual) and sums it with the input (identity). With the residual connection, the network not only keeps the gradient of the input as it goes deeper, but also it learns the residuals to be the same as the input. Empirical evidence demonstrates that ResNet could be trained up to $1000$ layers. 
% \todo{figure}

\paragraph{Inception}
\label{model.inception}
Instead of only deepening, Szegedy \etal \cite{Szegedy2015} design a network by widening the architecture. For each layer, the network uses three different filter size (i.e., $1 \times 1$, $3 \times 3$, $5 \times 5$) and $3 \times 3$ max pooling layer. The overall network is designed to be upto $22$ layers. This design overcomes the scaling issue of the objects within the image. The next version of the paper, named \textit{InceptionV2} \cite{Szegedy2016}, considers factorizing the receptive fields such that $n \times n$ filter is reformulated as the stack of $1 \times n$ and $n \times 1$ filters, found to be $33 \%$ cheaper. The third version of the network utilizes RMSProp \todo{Cite RMSProp}, $7\times7$ factorized filters, BatchNorm \cite{Ioffe2015} and label smoothing to avoid over-fitting. The final modification made to the network \cite{Szegedy2017} is to use residual blocks as proposed in \cite{He2015}.

% % % % % % % % %
% Detection     %    
% % % % % % % % %
\subsubsection{Detection Architectures}
\label{subsubsec:dl.approaches.cnn.detection}
Here we introduce \sota object detection strategies utilized in X-ray security imaging. 

\paragraph{Sliding Window-based CNN}
\label{model.detection.sw}
As shown in figure \ref{fig:region-based}a, this classical object detection approach consists of two main stages: (i) object proposal (ii) object classification. The first stage generates objects of interests via a fixed sized $ n\times n $ window slides over the image horizontally and vertically. One issue of using a fixed size window is large objects within the image does not fit within the frame. To overcome this issue, a common practice in the literature is to use image pyramids by a multi-scale sampling of the image and subsequent image interpolation of window regions at differing scale to a fixed size classification region input size. 

\paragraph{Faster Region-based CNN (F-RCNN)}
\label{model.detection.frcnn}
Proposed by Ren \etal \cite{Ren2015}, and depicted in figure \ref{fig:region-based}, F-RCNN is designed to have two sub-networks: (i) Region Proposal Network and (ii) Fast RCNN network \cite{Girshick2015}. RPN network generates objects of interests with varying anchors by sliding a $3 \times 3$ window through the convolutional feature map, shared with the Fast RCNN sub-network (figure \ref{fig:region-based}b).  Based on the feature map from the convolutional layer, a set of fully connected layers predicts the bounding box and objectness score of the region (\textit{an object} or \textit{background}). The Region of Interest (RoI) pooling layer then resizes the regions of interests generated by the RPN with varying aspect ratios. $ fc $ layers then create the final feature map to be used by bounding box regression and softmax layers.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\columnwidth]{img/frcnn.pdf}
%     \caption{Faster RCNN network \cite{Ren2015}.}
%     \label{fig:faster.rcnn}
% \end{figure}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\columnwidth]{img/rfcn.pdf}
%     % \missingfigure[]{R-FCN network}
%     \caption{Region-based fully convolutional neural network (R-FCN), proposed by \cite{Ren2015}, removes fully-connected $fc$ layers from F-RCNN to accelerate training.}
%     \label{fig:rfcn}
% \end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{img/region-based.pdf}
    % \missingfigure[]{R-FCN network}
    \caption{Region-based fully convolutional neural network (R-FCN), proposed by \cite{Ren2015}, removes fully-connected $fc$ layers from F-RCNN to accelerate training.}
    \label{fig:region-based}
\end{figure}

\paragraph{Region-based Fully CNN  (R-FCN)}
\label{model.detection.rfcn}
Proposed by Dai et al. \cite{Dai2016b}, R-FCN removes the $fc$ layers from F-RCNN to accelerate the training. The use of $fc$ layers in F-RCNN leads to multiple computations of the region proposals, which is rather expensive (figure \ref{fig:region-based}c). Instead of using $fc$ layers, R-FCN employs convolutional layers, and a unique scoring map, called \textit{position sensitive scoring map} \cite{Dai2016b}, which achieves the similar performance much more efficiently. 

\paragraph{RetinaNet}
\label{model.detection.retinanet}
Despite the speed, the downside of single-shot detection algorithms is the poorer detection performance compared to region-based approaches. Another issue is the imbalanced class size as the number of background samples is significantly higher than objects of interests, which adversely dominates the loss. RetinaNet addresses these issues and is based on two main contributions: (i) Feature Pyramid Networks (FPN), (ii) Focal Loss. The notion of FPN is somewhat similar to UNet \cite{Ronneberger2015}, whereby high-level features (first layers) and low-level (higher layers) feature maps are combined.  The advantage of using focal loss during training is the elimination of class imbalance posed by a large number of background samples. Focal-loss weights the well-classified samples for the objective function to focus more on hard and interesting examples to learn. Hence the proposed method addresses the issues of the single-shot methods and achieves comparable performance to region-based detection approaches. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{img/single-shot.pdf}
    % \missingfigure[]{SSD}
    \caption{The pipeline of the Single Shot Multi-Box Detector.}
    \label{fig:single.shot}
\end{figure}


\paragraph{Single Shot Multi-Box Detector (SSD)}
\label{model.detection.ssd}
As the name suggests, this approach performs object detection with single forward-pass, without needing for another region proposal sub-network. The architecture utilizes a \hyperref[model.vgg]{VGG} network by replacing its $fc$ layers with convolutional layers, which helps to extract features from multiple scales, and also to reduce the size of the output for the next layer. The approach splits the input image into $4 \times 4$ and $8 \times 8$ feature maps, whereby six manually configured bounding boxes are predicted per feature map cell. The objective of the architecture is to optimize a loss function that combines objectness loss and bounding box location loss, computed via a cross-entropy and $\mathcal{L}_1$ losses, respectively. The proposed approach yields statistically reliable and computationally efficient results. 

% \ssection{YOLO}
\paragraph{YOLO}
\label{model.detection.yolo}
Similar to \hyperref[model.detection.ssd]{SSD}, Redmon \etal \cite{Redmon2016} also propose a fully convolutional object detection network that needs only one forward-pass (figure \ref{fig:single.shot}b). Similar to Faster RCNN, YOLO also utilizes several anchors to handle the objects with varying aspect ratios. Unlike Faster RCNN that uses fixed size anchors, however, YOLO clusters the ground-truth bounding boxes via 
\textit{k}-means clustering to learn the data specific anchor parameters. Minor modifications to the approach such as BatchNorm and the use of higher resolution input images together with multi-scale training yield better detection performance. For instance, the network can train images of sizes that range between  $350\times350$ to $600\times600$. It divides the input into $13\times13$ grid cells, each of which predicts $5$ bounding box coordinates for each anchor. Moreover, for individual predicted bounding boxes, the network outputs confidence score showing the similarity between the bounding boxes and the ground truth. Finally, the output also includes the probability distribution of the classes that the predicted bounding boxes belong. 


% % % % % % % % %
% Segmentation     %    
% % % % % % % % %
\subsubsection{Segmentation Architectures}
\label{subsubsec:dl.approaches.cnn.segmentation}
The use of segmentation approaches in X-ray security imaging is limited due to the expense of collecting large segmentation datasets. Recently, there are few recent research applying segmentation algorithms within this domain. Here, we introduce the current \sota instance segmentation algorithm, utilized within the recent research.

\paragraph{Mask-RCNN}
\label{model.segmentation.mask.rcnn}
Proposed by He \etal \cite{He2017}, Mask-RCNN is an instance segmentation algorithm that simultaneously performs detection and segmentation to each object within an image. The proposed approach is composed of two main stages and utilizes two well-established detection and segmentation algorithms. The first stage uses \hyperref[model.detection.frcnn]{F-RCNN} detection strategy to perform object detection via the box regression and classification layers (figure \ref{fig:region-based}b). The second stage is the \textit{mask branch} that is a binary mask classifier that classifies each pixel within a bounding box as a target class (cat, dog, etc.) or background. Combining binary mask classifier with F-RCNN (figure \ref{fig:mask-rcnn}) detection module yields \sota instance segmentation results. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{img/mask-rcnn.pdf}
    \caption{Mask-RCNN pipeline. The architecture simultaneously performs detection and instance segmentation.}
    \label{fig:mask-rcnn}
\end{figure}



\subsection{Unsupervised CNN Architectures}
\label{dl.approaches.unsupervised}
Previous approaches introduced in Section \ref{subsubsec:dl.approaches.cnn} are supervised learning techniques such that the input dataset contains ground-truth labels, and the model is trained to predict the labels. In some applications, however, the ground-truth labels are not available within the dataset, also known as unsupervised learning. This section introduces unsupervised learning approaches 

\subsubsection{Autoencoders}
\label{dl.approaches.autoencoder}
An autoencoder is an unsupervised neural network that encodes an input $x$ to a lower-dimensional latent space $z$, then reconstructs the input from the latent space via a decoder network (figure \ref{fig:autoencoder}). 
\begin{figure}[ht]
    \centering
    \includegraphics{img/autoencoder.pdf}
    \caption{An autoencoder pipeline}
    \label{fig:autoencoder}
\end{figure}
The objective here is to learn a model that is capable of reconstructing the output $\hat{x}$ as close to input $x$ as possible. Hence, the optimization problem becomes
\begin{equation}
    \mathcal{L} = \argmin_{\Theta} |x - \hat{x}|.   
\end{equation}



\subsubsection{Generative Adversarial Networks (GAN)}
\label{dl.approaches.gan}
Initially proposed by Goodfellow \etal \cite{Goodfellow2014}, GAN is unsupervised deep neural architectures that learn to capture any input data distribution by predicting features from an initially hidden representation $z$. The theory behind GAN is based on a competition between the two networks within a zero-sum game framework, as initially used in game theory. The first network, called \textit{Generator} ($G$), aims to generate high dimensional output from a low-dimension latent space, which is commonly a random noise vector. The use of a decoder-alike network architecture upsamples the latent vector to a higher-dimensional feature map. The second network, called \textit{Discriminator} ($D$), measures the similarity between the original input (\textit{real}) and the generated output (\textit{fake}). The discriminator network usually adopts an encoder network architecture such that for a given high-dimensional feature, it predicts its class label. The objective during the training is that the generator aims to produce as realistic output as possible, while the discriminator tries to classify the two images as \textit{real correctly} or \textit{fake}. With optimization based on a zero-sum game framework, each network strengthens its prediction capability until they reach an equilibrium. The task here, hence, is the minimization and the maximization of $G$ and $D$, respectively. The overall loss function for this objective is as follows:

\begin{equation}
    \underset{G}{\text{min }} \underset{D}{\text{max }} \underset{x \sim p_x}{\mathbb{E}} [\log D(x)] + \underset{z \sim p_z}{\mathbb{E}} [\log (1-D(G(z))].
\end{equation}

\begin{figure}[ht]
    \centering
    \includegraphics{img/gan.pdf}
    % \missingfigure[]{GAN figure.}
    \caption{A generative adversarial network }
    \label{fig:gan}
\end{figure}


